High fidelity simulations of unstart phenomena in a scramjet inlet due to angle of attack

This work investigates the unsteady behavior of unstart phenomena within a scramjet inlet using advanced computational techniques. Scramjets and ramjets, with their reliance on inlet compression, offer promising airbreathing propulsion for hypersonic regimes. This research focuses on understanding and modeling the onset of unstart phenomena in supersonic inlets, a critical step towards developing mitigation strategies. These strategies have the potential to improve engine efficiency, range, and maneuverability of hypersonic vehicles. To achieve this, the state-of-the-art compressible flow solver, Eilmer, is used to simulate shockwave behavior within the inlet/isolator of a planar scramjet characterized experimentally at North Carolina State University (NCSU). Baseline comparisons are presented with the wind tunnel experiments via the shock structures present within the isolator section conducted at Mach 3.9 on a 3D scramjet inlet model. Simulations are then carried out at varying angles of attack (0 to 10 deg) and multiple pitch rates (10 deg/sec and 100 deg/sec) to demonstrate the shock train inertial response and to characterize unstart onset. In both cases the timing of inlet unstart is observed to correlate well with the rapid surge in exit pressure as well as shock detachment at the lower leading edge region. Lastly, exit pressures are significantly higher in the 10 deg/s case than in that of the 100 deg/s case at the same angle of attack. These observations suggest that unstart is not only dependent on angle of attack but also on AoA pitch rate. The findings provide valuable insights into the unsteady flow behavior during hypersonic inlet unstart, with potential applications for unstart detection at high angles of attack.

==> 01abstract.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Abstract:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%This work investigates the unsteady behavior of unstart phenomena in a scramjet/ramjet inlet, to enhance hypersonic flight capabilities. Scramjets and ramjets, with their unique inlet-based compression mechanisms, hold promise for airbreathing propulsion in supersonic and hypersonic regimes. Understanding and modeling the onset of unstart phenomena in supersonic inlets could expand the flight envelope, by developing mitigation strategies leading to improved efficiency, range, and maneuverability. To fully explore these theoretical benefits, this study employs Eilmer, a state-of-the-art massively paralleled compressible Navier-Stokes solver with thermochemical non-equilibrium and turbulence modeling capabilties. Reynolds Average Navier Stokes (RANS) turbulence models based on finite volume formulation with a Spalart Almaras method was employed to investigate the shocktrain dynamics during unstart. Inlet flow physics is experimentally validated at Mach 3.9 using the North Carolina State University (NCSU) wind tunnel facility that is equipped with a 3D scramjet inlet/isolator model with a shock on lip design condition at Mach 2.5 and a physical area contraction ratio, CR, 2.64. This is following by simulations at varying angles of attack (AoA) at three speeds to fully characterize the onset of unstart dynamics. The results provide valuable insights into the unsteady characteristics and flow evolution of hypersonic inlet unstart and provide potential practical applications on its detection under high AoA. 

% This work investigates the unsteady behavior of unstart phenomena within a scramjet inlet using advanced computational techniques. Scramjets and ramjets, with their reliance on inlet compression, offer promising airbreathing propulsion for hypersonic regimes. This research focuses on understanding and modeling the onset of unstart phenomena in supersonic inlets, a critical step towards developing mitigation strategies. These strategies have the potential to improve engine efficiency, range, and maneuverability of hypersonic vehicles. To achieve this, the state-of-the-art compressible flow solver, Eilmer, is used to simulate shockwave behavior within the inlet/isolator of a planar scramjet characterized experimentally at North Carolina State University (NCSU). The simulations employ the classical Spalart Almaras, Reynolds Averaged Navier-Stokes (RANS), turbulence model to capture the dynamics of shockwaves during unstart. Baseline comparisons are presented with the wind tunnel experiments via the shock structures present within the isolator section conducted at Mach 3.9 on a 3D scramjet inlet model. Simulations are then carried out at varying angles of attack (0 to 10 deg) and multiple pitch rates (10 deg/sec and 100 deg/sec) to demonstrate the shock train inertial response and to characterize unstart onset comprehensively. In both cases the timing of inlet unstart is observed to correlate well with the rapid surge in exit pressure as well as shock detachment at the lower leading edge region. Lastly, exit pressures are significantly higher in the 10 deg/s case than in that of the 100 deg/s case at the same angle of attack. These observations suggest that unstart is not only dependent on angle of attack but also on AoA pitch rate. The findings provide valuable insights into the unsteady flow behavior during hypersonic inlet unstart, with potential applications for unstart detection at high angles of attack.

%This work is in direct support of  the “Surface Morphing and Adaptive Structures for Hypersonics (SMASH)” currently pursued by DEVCOM - Army Research Laboratory in collaboration with NRL (Naval Research Laboratory), AFRL (Air Force Research Laboratory) and MDA (Missile Defense Agency) under the sponsorship of OUSD (Office of the Under Secretary of Defense).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
